GP+: A Python Library for Kernel-based learning via Gaussian Processes

In this paper we introduce GP+, an open-source library for kernel-based learning via Gaussian processes (GPs) which are powerful statistical models that are completely characterized by their parametric covariance and mean functions. GP+ is built on PyTorch and provides a user-friendly and object-oriented tool for probabilistic learning and inference. As we demonstrate with a host of examples, GP+ has a few unique advantages over other GP modeling libraries. We achieve these advantages primarily by integrating nonlinear manifold learning techniques with GPs' covariance and mean functions. As part of introducing GP+, in this paper we also make methodological contributions that (1) enable probabilistic data fusion and inverse parameter estimation, and (2) equip GPs with parsimonious parametric mean functions which span mixed feature spaces that have both categorical and quantitative variables. We demonstrate the impact of these contributions in the context of Bayesian optimization, multi-fidelity modeling, sensitivity analysis, and calibration of computer models.

==> 01_Ref.tex <==
@article{RN791,
   author = {Zhang, W. Z. and Bostanabad, R. and Liang, B. and Su, X. M. and Zeng, D. and Bessa, M. A. and Wang, Y. C. and Chen, W. and Cao, J.},
   title = {A numerical Bayesian-calibrated characterization method for multiscale prepreg preforming simulations with tension-shear coupling},
   journal = {Composites Science and Technology},
   volume = {170},
   pages = {15-24},
   ISSN = {0266-3538},
   DOI = {10.1016/j.compscitech.2018.11.019},
   url = {<Go to ISI>://WOS:000456228100003},
   year = {2019},
   type = {Journal Article}
}

@article{RN645,
   author = {Bayarri, Maria J. and Berger, James O. and Paulo, Rui and Sacks, Jerry and Cafeo, John A. and Cavendish, James and Lin, Chin-Hsu and Tu, Jian},
   title = {A Framework for Validation of Computer Models},
   journal = {Technometrics},
   volume = {49},
   number = {2},
   pages = {138-154},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1198/004017007000000092},
   url = {<Go to ISI>://WOS:000246053000003},
   year = {2007},
   type = {Journal Article}
}

@article{RN270,
   author = {Higdon, Dave and Kennedy, Marc and Cavendish, James C. and Cafeo, John A. and Ryne, Robert D.},
   title = {Combining Field Data and Computer Simulations for Calibration and Prediction},
   journal = {SIAM Journal on Scientific Computing},
   volume = {26},
   number = {2},
   pages = {448-466},
   ISSN = {1064-8275
1095-7197},
   DOI = {10.1137/s1064827503426693},
   url = {<Go to ISI>://WOS:000226823100006},
   year = {2004},
   type = {Journal Article}
}




@article{oune2021latent,
  title={Latent map Gaussian processes for mixed variable metamodeling},
  author={Oune, Nicholas and Bostanabad, Ramin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={387},
  pages={114128},
  year={2021},
  publisher={Elsevier}
}

@article{bostanabad2018leveraging,
  title={Leveraging the nugget parameter for efficient Gaussian process modeling},
  author={Bostanabad, Ramin and Kearney, Tucker and Tao, Siyu and Apley, Daniel W and Chen, Wei},
  journal={International journal for numerical methods in engineering},
  volume={114},
  number={5},
  pages={501--516},
  year={2018},
  publisher={Wiley Online Library}
}

@article{RN783,
   author = {Bostanabad, R. and Kearney, T. and Tao, S. Y. and Apley, D. W. and Chen, W.},
   title = {Leveraging the nugget parameter for efficient Gaussian process modeling},
   journal = {International Journal for Numerical Methods in Engineering},
   volume = {114},
   number = {5},
   pages = {501-516},
   ISSN = {0029-5981},
   DOI = {10.1002/nme.5751},
   url = {<Go to ISI>://WOS:000428998100002},
   year = {2018},
   type = {Journal Article}
}
@inproceedings{RN649,
   author = {Tao, Siyu and Shintani, Kohei and Bostanabad, Ramin and Chan, Yu-Chin and Yang, Guang and Meingast, Herb and Chen, Wei},
   title = {Enhanced Gaussian Process Metamodeling and Collaborative Optimization for Vehicle Suspension Design Optimization},
   booktitle = {ASME 2017 International Design Engineering Technical Conferences and Computers and Information in Engineering Conference},
   publisher = {American Society of Mechanical Engineers},
   volume = {2B},
   type = {Conference Proceedings}
}


@article{kennedy2001bayesian,
  title={Bayesian calibration of computer models},
  author={Kennedy, Marc C and O'Hagan, Anthony},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={63},
  number={3},
  pages={425--464},
  year={2001},
  publisher={Wiley Online Library}
}

@article{seeger2004gaussian,
  title={Gaussian processes for machine learning},
  author={Seeger, Matthias},
  journal={International journal of neural systems},
  volume={14},
  number={02},
  pages={69--106},
  year={2004},
  publisher={World Scientific}
}

@article{bostanabad2019globally,
  title={Globally approximate gaussian processes for big data with application to data-driven metamaterials design},
  author={Bostanabad, Ramin and Chan, Yu-Chin and Wang, Liwei and Zhu, Ping and Chen, Wei},
  journal={Journal of Mechanical Design},
  volume={141},
  number={11},
  pages={111402},
  year={2019},
  publisher={American Society of Mechanical Engineers}
}

@book{gramacy2020surrogates,
  title={Surrogates: Gaussian process modeling, design, and optimization for the applied sciences},
  author={Gramacy, Robert B},
  year={2020},
  publisher={CRC press}
}

@article{eweis2022data,
  title={Data fusion with latent map Gaussian processes},
  author={Eweis-Labolle, Jonathan Tammer and Oune, Nicholas and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  volume={144},
  number={9},
  pages={091703},
  year={2022},
  publisher={American Society of Mechanical Engineers}
}

@article{yousefpour2023unsupervised,
  title={Unsupervised Anomaly Detection via Nonlinear Manifold Learning},
  author={Yousefpour, Amin and Shishehbor, Mehdi and Foumani, Zahra Zanjani and Bostanabad, Ramin},
  journal={arXiv preprint arXiv:2306.09441},
  year={2023}
}

@book{rasmussen2006gaussian,
  title={Gaussian processes for machine learning},
  author={Rasmussen, Carl Edward and Williams, Christopher KI and others},
  volume={1},
  year={2006},
  publisher={Springer}
}

@article{foumani2023multi,
  title={Multi-fidelity cost-aware Bayesian optimization},
  author={Foumani, Zahra Zanjani and Shishehbor, Mehdi and Yousefpour, Amin and Bostanabad, Ramin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={407},
  pages={115937},
  year={2023},
  publisher={Elsevier}
}

@article{RN1392,
   author = {Balandat, Maximilian and Karrer, Brian and Jiang, Daniel and Daulton, Samuel and Letham, Ben and Wilson, Andrew G. and Bakshy, Eytan},
   title = {BoTorch: A framework for efficient Monte-Carlo Bayesian optimization},
   journal = {Advances in Neural Information Processing Systems},
   volume = {33},
   year = {2020},
   type = {Journal Article}
}

@article{RN1270,
   author = {Gardner, Jacob R. and Pleiss, Geoff and Bindel, David and Weinberger, Kilian Q. and Wilson, Andrew Gordon},
   title = {Gpytorch: Blackbox matrix-matrix gaussian process inference with gpu acceleration},
   journal = {arXiv preprint arXiv:1809.11165},
   year = {2018},
   type = {Journal Article}
}
@article{RN1790,
   author = {Renganathan, S Ashwin and Rao, Vishwas and Navon, Ionel M},
   title = {CAMERA: A Method for Cost-aware, Adaptive, Multifidelity, Efficient Reliability Analysis},
   journal = {arXiv preprint arXiv:2203.01436},
   year = {2022},
   type = {Journal Article}
}


@article{frazier2008knowledge,
  title={A knowledge-gradient policy for sequential information collection},
  author={Frazier, Peter I and Powell, Warren B and Dayanik, Savas},
  journal={SIAM Journal on Control and Optimization},
  volume={47},
  number={5},
  pages={2410--2439},
  year={2008},
  publisher={SIAM}
}

@article{balandat2020botorch,
  title={BoTorch: a framework for efficient Monte-Carlo Bayesian optimization},
  author={Balandat, Maximilian and Karrer, Brian and Jiang, Daniel and Daulton, Samuel and Letham, Ben and Wilson, Andrew G and Bakshy, Eytan},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={21524--21538},
  year={2020}
}

@Misc{gpy2014,
  author =   {{GPy}},
  title =    {{GPy}: A Gaussian process framework in python},
  howpublished = {\url{http://github.com/SheffieldML/GPy}},
  year = {since 2012}
}

@article{gardner2018gpytorch,
  title={Gpytorch: Blackbox matrix-matrix gaussian process inference with gpu acceleration},
  author={Gardner, Jacob and Pleiss, Geoff and Weinberger, Kilian Q and Bindel, David and Wilson, Andrew G},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@article{matthews2017gpflow,
  title={GPflow: A Gaussian Process Library using TensorFlow.},
  author={Matthews, Alexander G de G and Van Der Wilk, Mark and Nickson, Tom and Fujii, Keisuke and Boukouvalas, Alexis and Le{\'o}n-Villagr{\'a}, Pablo and Ghahramani, Zoubin and Hensman, James},
  journal={J. Mach. Learn. Res.},
  volume={18},
  number={40},
  pages={1--6},
  year={2017}
}

@phdthesis{moon2010design,
  title={Design and analysis of computer experiments for screening input variables},
  author={Moon, Hyejung},
  year={2010},
  school={The Ohio State University}
}

@article{planas2021evolutionary,
  title={Evolutionary gaussian processes},
  author={Planas, Robert and Oune, Nick and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  volume={143},
  number={11},
  pages={111703},
  year={2021},
  publisher={American Society of Mechanical Engineers}
}

@article{gramacy2007tgp,
  title={tgp: an R package for Bayesian nonstationary, semiparametric nonlinear regression and design by treed Gaussian process models},
  author={Gramacy, Robert B},
  journal={Journal of Statistical Software},
  volume={19},
  pages={1--46},
  year={2007}
}

@article{harkonen2022mixtures,
  title={Mixtures of Gaussian Process Experts with  $SMC^2$},
  author={H{\"a}rk{\"o}nen, Teemu and Wade, Sara and Law, Kody and Roininen, Lassi},
  journal={arXiv preprint arXiv:2208.12830},
  year={2022}
}

@inproceedings{candelieri2021treed,
  title={Treed-gaussian processes with support vector machines as nodes for nonstationary Bayesian optimization},
  author={Candelieri, Antonio and Pedrielli, Giulia},
  booktitle={2021 Winter Simulation Conference (WSC)},
  pages={1--12},
  year={2021},
  organization={IEEE}
}
@inproceedings{bitzer2023hierarchical,
  title={Hierarchical-Hyperplane Kernels for Actively Learning Gaussian Process Models of Nonstationary Systems},
  author={Bitzer, Matthias and Meister, Mona and Zimmer, Christoph},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={7897--7912},
  year={2023},
  organization={PMLR}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@article{chipman1998bayesian,
  title={Bayesian CART model search. Commentaries. Authors' reply},
  author={Chipman, HA and George, EI and McCulloch, RE and ZHANG, H and KNIGHT, K and KUSTRA, R},
  journal={Journal of the American Statistical Association},
  volume={93},
  number={443},
  pages={935--960},
  year={1998}
}

@article{bostanabad2018leveraging,
  title={Leveraging the nugget parameter for efficient Gaussian process modeling},
  author={Bostanabad, Ramin and Kearney, Tucker and Tao, Siyu and Apley, Daniel W and Chen, Wei},
  journal={International journal for numerical methods in engineering},
  volume={114},
  number={5},
  pages={501--516},
  year={2018},
  publisher={Wiley Online Library}
}

@article{macdonald2015gpfit,
  title={GPfit: An R package for fitting a Gaussian process model to deterministic simulator outputs},
  author={MacDonald, Blake and Ranjan, Pritam and Chipman, Hugh},
  journal={Journal of Statistical Software},
  volume={64},
  pages={1--23},
  year={2015}
}

@article{sacks1989mitchell,
  title={Mitchell, and HP Wynn,“Design and analysis of computer experiments,”},
  author={Sacks, WJ and Welch, TJ},
  journal={Statistical Science},
  volume={4},
  number={4},
  pages={409--453},
  year={1989}
}

@article{gramacy2012cases,
  title={Cases for the nugget in modeling computer experiments},
  author={Gramacy, Robert B and Lee, Herbert KH},
  journal={Statistics and Computing},
  volume={22},
  pages={713--722},
  year={2012},
  publisher={Springer}
}

@article{sobol1990sensitivity,
  title={On sensitivity estimation for nonlinear mathematical models},
  author={Sobol', Il'ya Meerovich},
  journal={Matematicheskoe modelirovanie},
  volume={2},
  number={1},
  pages={112--118},
  year={1990},
  publisher={Russian Academy of Sciences, Branch of Mathematical Sciences}
}

@article{egger2016hybrid,
  title={Hybrid organic--inorganic perovskites on the move},
  author={Egger, David A and Rappe, Andrew M and Kronik, Leeor},
  journal={Accounts of chemical research},
  volume={49},
  number={3},
  pages={573--581},
  year={2016},
  publisher={ACS Publications}
}

@article{wolpert2010conditional,
  title={Conditional expectation},
  author={Wolpert, Robert L},
  journal={University Lecture},
  year={2010}
}

@book{rudary2009predictive,
  title={On predictive linear gaussian models},
  author={Rudary, Matthew R},
  year={2009},
  publisher={University of Michigan}
}

@article{rao2022machine,
  title={Machine learning--enabled high-entropy alloy discovery},
  author={Rao, Ziyuan and Tung, Po-Yen and Xie, Ruiwen and Wei, Ye and Zhang, Hongbin and Ferrari, Alberto and Klaver, TPC and K{\"o}rmann, Fritz and Sukumar, Prithiv Thoudden and Kwiatkowski da Silva, Alisson and others},
  journal={Science},
  volume={378},
  number={6615},
  pages={78--85},
  year={2022},
  publisher={American Association for the Advancement of Science}
}


@article{tao2021latent,
  title={Latent variable Gaussian process models: A rank-based analysis and an alternative approach},
  author={Tao, Siyu and Apley, Daniel W and Plumlee, Matthew and Chen, Wei},
  journal={International Journal for Numerical Methods in Engineering},
  volume={122},
  number={15},
  pages={4007--4026},
  year={2021},
  publisher={Wiley Online Library}
}

@article{poloczek2017multi,
  title={Multi-information source optimization},
  author={Poloczek, Matthias and Wang, Jialei and Frazier, Peter},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{bonilla2007multi,
  title={Multi-task Gaussian process prediction},
  author={Bonilla, Edwin V and Chai, Kian and Williams, Christopher},
  journal={Advances in neural information processing systems},
  volume={20},
  year={2007}
}

@misc{RN1576,
   volume = {97},
   pages = {354--363},
   url = {https://proceedings.mlr.press/v97/astudillo19a.html},
   year = {2019},
   type = {Conference Paper}
}

@article{RN578,
   author = {Balachandran, P. V. and Xue, D. and Theiler, J. and Hogden, J. and Lookman, T.},
   title = {Adaptive Strategies for Materials Design using Uncertainties},
   journal = {Sci Rep},
   volume = {6},
   pages = {19660},
   ISSN = {2045-2322 (Electronic)
2045-2322 (Linking)},
   DOI = {10.1038/srep19660},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/26792532},
   year = {2016},
   type = {Journal Article}
}

@article{RN1392,
   author = {Balandat, Maximilian and Karrer, Brian and Jiang, Daniel and Daulton, Samuel and Letham, Ben and Wilson, Andrew G. and Bakshy, Eytan},
   title = {BoTorch: A framework for efficient Monte-Carlo Bayesian optimization},
   journal = {Advances in Neural Information Processing Systems},
   volume = {33},
   year = {2020},
   type = {Journal Article}
}

@article{RN1632,
   author = {Herbol, Henry C and Poloczek, Matthias and Clancy, Paulette},
   title = {Cost-effective materials discovery: Bayesian optimization across multiple information sources},
   journal = {Materials Horizons},
   volume = {7},
   number = {8},
   pages = {2113-2123},
   year = {2020},
   type = {Journal Article}
}

@article{RN1242,
   author = {Kusne, A. G. and Yu, H. and Wu, C. and Zhang, H. and Hattrick-Simpers, J. and DeCost, B. and Sarker, S. and Oses, C. and Toher, C. and Curtarolo, S. and Davydov, A. V. and Agarwal, R. and Bendersky, L. A. and Li, M. and Mehta, A. and Takeuchi, I.},
   title = {On-the-fly closed-loop materials discovery via Bayesian active learning},
   journal = {Nat Commun},
   volume = {11},
   number = {1},
   pages = {5966},
   ISSN = {2041-1723 (Electronic)
2041-1723 (Linking)},
   DOI = {10.1038/s41467-020-19597-w},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/33235197},
   year = {2020},
   type = {Journal Article}
}

@inproceedings{RN1789,
   author = {Takeno, Shion and Fukuoka, Hitoshi and Tsukada, Yuhki and Koyama, Toshiyuki and Shiga, Motoki and Takeuchi, Ichiro and Karasuyama, Masayuki},
   title = {Multi-fidelity Bayesian optimization with max-value entropy search and its parallelization},
   booktitle = {International Conference on Machine Learning},
   publisher = {PMLR},
   pages = {9334-9345},
   ISBN = {2640-3498},
   type = {Conference Proceedings}
}

@article{RN1794,
   author = {Tran, Anh and Tranchida, Julien and Wildey, Tim and Thompson, Aidan P.},
   title = {Multi-fidelity machine-learning with uncertainty quantification and Bayesian optimization for materials design: Application to ternary random alloys},
   journal = {The Journal of Chemical Physics},
   volume = {153},
   number = {7},
   pages = {074705},
   DOI = {10.1063/5.0015672},
   url = {https://aip.scitation.org/doi/abs/10.1063/5.0015672},
   year = {2020},
   type = {Journal Article}
}

@article{RN1761,
   author = {Wang, Yifan and Chen, Tai-Ying and Vlachos, Dionisios G},
   title = {NEXTorch: a design and Bayesian optimization toolkit for chemical sciences and engineering},
   journal = {Journal of Chemical Information and Modeling},
   volume = {61},
   number = {11},
   pages = {5312-5319},
   ISSN = {1549-9596},
   year = {2021},
   type = {Journal Article}
}

@misc{RN1577,
   volume = {115},
   pages = {788--798},
   url = {https://proceedings.mlr.press/v115/wu20a.html},
   year = {2020},
   type = {Conference Paper}
}

@article{RN1845,
   author = {Zanjani Foumani, Zahra and Shishehbor, Mehdi and Yousefpour, Amin and Bostanabad, Ramin},
   title = {Multi-fidelity cost-aware Bayesian optimization},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {407},
   pages = {115937},
   ISSN = {0045-7825},
   DOI = {https://doi.org/10.1016/j.cma.2023.115937},
   url = {https://www.sciencedirect.com/science/article/pii/S0045782523000609},
   year = {2023},
   type = {Journal Article}
}

@article{RN1375,
   author = {Zhang, Y. and Apley, D. W. and Chen, W.},
   title = {Bayesian Optimization for Materials Design with Mixed Quantitative and Qualitative Variables},
   journal = {Sci Rep},
   volume = {10},
   number = {1},
   pages = {4924},
   ISSN = {2045-2322 (Electronic)
2045-2322 (Linking)},
   DOI = {10.1038/s41598-020-60652-9},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/32188873},
   year = {2020},
   type = {Journal Article}
}

@article{RN1881,
   author = {Batlle, Pau and Darcy, Matthieu and Hosseini, Bamdad and Owhadi, Houman},
   title = {Kernel methods are competitive for operator learning},
   journal = {arXiv preprint arXiv:2304.13202},
   year = {2023},
   type = {Journal Article}
}

@article{RN1886,
   author = {Chen, Yifan and Hosseini, Bamdad and Owhadi, Houman and Stuart, Andrew M},
   title = {Solving and learning nonlinear PDEs with Gaussian processes},
   journal = {Journal of Computational Physics},
   volume = {447},
   pages = {110668},
   ISSN = {0021-9991},
   year = {2021},
   type = {Journal Article}
}

@article{RN1890,
   author = {Meng, Rui and Yang, Xianjin},
   title = {Sparse Gaussian processes for solving nonlinear PDEs},
   journal = {Journal of Computational Physics},
   volume = {490},
   pages = {112340},
   ISSN = {0021-9991},
   year = {2023},
   type = {Journal Article}
}

@article{RN272,
   author = {Arendt, Paul D. and Apley, Daniel W. and Chen, Wei},
   title = {Quantification of Model Uncertainty: Calibration, Model Discrepancy, and Identifiability},
   journal = {Journal of Mechanical Design},
   volume = {134},
   number = {10},
   pages = {100908},
   ISSN = {1050-0472
1528-9001},
   DOI = {10.1115/1.4007390},
   url = {<Go to ISI>://WOS:000309654400010},
   year = {2012},
   type = {Journal Article}
}

@article{RN271,
   author = {Arendt, Paul D and Apley, Daniel W and Chen, Wei and Lamb, David and Gorsich, David},
   title = {Improving identifiability in model calibration using multiple responses},
   journal = {Journal of Mechanical Design},
   volume = {134},
   number = {10},
   pages = {100909},
   ISSN = {1050-0472},
   year = {2012},
   type = {Journal Article}
}

@article{RN337,
   author = {Bayarri, M. J. and Berger, J. O. and Liu, F.},
   title = {Modularization in Bayesian analysis, with emphasis on analysis of computer
 models},
   journal = {Bayesian Analysis},
   volume = {4},
   number = {1},
   pages = {119-150},
   ISSN = {1936-0975},
   DOI = {10.1214/09-ba404},
   url = {<Go to ISI>://WOS:000273483200008},
   year = {2009},
   type = {Journal Article}
}

@article{RN705,
   author = {Kennedy, Marc C and O'Hagan, Anthony},
   title = {Bayesian calibration of computer models},
   journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
   volume = {63},
   number = {3},
   pages = {425-464},
   ISSN = {1467-9868},
   year = {2001},
   type = {Journal Article}
}

@article{RN334,
   author = {Loeppky, J and Bingham, Derek and Welch, W},
   title = {Computer model calibration or tuning in practice},
   journal = {Technometrics, submitted for publication},
   year = {2006},
   type = {Journal Article}
}

@book{RN841,
   author = {Smith, Ralph C},
   title = {Uncertainty quantification: theory, implementation, and applications},
   publisher = {Siam},
   volume = {12},
   ISBN = {161197321X},
   year = {2013},
   type = {Book}
}

@article{RN1275,
   author = {Cutajar, Kurt and Pullin, Mark and Damianou, Andreas and Lawrence, Neil and González, Javier},
   title = {Deep gaussian processes for multi-fidelity modeling},
   journal = {arXiv preprint arXiv:1903.07320},
   year = {2019},
   type = {Journal Article}
}

@article{RN1266,
   author = {Fernández-Godino, M. Giselle and Park, Chanyoung and Kim, Nam-Ho and Haftka, Raphael T.},
   title = {Review of multi-fidelity models},
   journal = {arXiv preprint arXiv:1609.07196},
   year = {2016},
   type = {Journal Article}
}

@article{RN1786,
   author = {Deng, Shiguang and Mora, Carlos and Apelian, Diran and Bostanabad, Ramin},
   title = {Data-Driven Calibration of Multifidelity Multiscale Fracture Models Via Latent Map Gaussian Process},
   journal = {Journal of Mechanical Design},
   volume = {145},
   number = {1},
   pages = {1-15},
   ISSN = {1050-0472
1528-9001},
   DOI = {10.1115/1.4055951},
   url = {https://doi.org/10.1115/1.4055951},
   year = {2023},
   type = {Journal Article}
}

@article{RN1838,
   author = {Eweis-Labolle, Jonathan Tammer and Oune, Nicholas and Bostanabad, Ramin},
   title = {Data Fusion With Latent Map Gaussian Processes},
   journal = {Journal of Mechanical Design},
   volume = {144},
   number = {9},
   ISSN = {1050-0472},
   DOI = {10.1115/1.4054520},
   url = {https://doi.org/10.1115/1.4054520},
   year = {2022},
   type = {Journal Article}
}

@article{RN1559,
   author = {Oune, N. and Bostanabad, R.},
   title = {Latent map Gaussian processes for mixed variable metamodeling},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {387},
   pages = {114128},
   ISSN = {0045-7825},
   DOI = {ARTN 114128
10.1016/j.cma.2021.114128},
   url = {<Go to ISI>://WOS:000708647400003},
   year = {2021},
   type = {Journal Article}
}

@article{RN1558,
   author = {Planas, R. and Oune, N. and Bostanabad, R.},
   title = {Evolutionary Gaussian Processes},
   journal = {Journal of Mechanical Design},
   volume = {143},
   number = {11},
   pages = {111703},
   ISSN = {1050-0472},
   DOI = {Artn 111703
10.1115/1.4050746},
   url = {<Go to ISI>://WOS:000702466200013},
   year = {2021},
   type = {Journal Article}
}

@article{RN791,
   author = {Zhang, W. Z. and Bostanabad, R. and Liang, B. and Su, X. M. and Zeng, D. and Bessa, M. A. and Wang, Y. C. and Chen, W. and Cao, J.},
   title = {A numerical Bayesian-calibrated characterization method for multiscale prepreg preforming simulations with tension-shear coupling},
   journal = {Composites Science and Technology},
   volume = {170},
   pages = {15-24},
   ISSN = {0266-3538},
   DOI = {10.1016/j.compscitech.2018.11.019},
   url = {<Go to ISI>://WOS:000456228100003},
   year = {2019},
   type = {Journal Article}
}

@inproceedings{RN718,
   author = {Damianou, Andreas and Lawrence, Neil},
   title = {Deep gaussian processes},
   booktitle = {Artificial Intelligence and Statistics},
   pages = {207-215},
   type = {Conference Proceedings}
}

@article{RN503,
   author = {Gramacy, Robert B. and Apley, Daniel W.},
   title = {Local Gaussian Process Approximation for Large Computer Experiments},
   journal = {Journal of Computational and Graphical Statistics},
   volume = {24},
   number = {2},
   pages = {561-578},
   ISSN = {1061-8600
1537-2715},
   DOI = {10.1080/10618600.2014.914442},
   url = {<Go to ISI>://WOS:000356365700013},
   year = {2015},
   type = {Journal Article}
}

@article{RN698,
   author = {Guhaniyogi, R. and Banerjee, S.},
   title = {Meta-Kriging: Scalable Bayesian Modeling and Inference for Massive Spatial Datasets},
   journal = {Technometrics},
   volume = {60},
   number = {4},
   pages = {430-444},
   ISSN = {0040-1706 (Print)
0040-1706 (Linking)},
   DOI = {10.1080/00401706.2018.1437474},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/31007296},
   year = {2018},
   type = {Journal Article}
}

@article{RN893,
   author = {Hensman, James and Fusi, Nicolo and Lawrence, Neil D},
   title = {Gaussian processes for big data},
   journal = {arXiv preprint arXiv:1309.6835},
   year = {2013},
   type = {Journal Article}
}

@article{RN1574,
   author = {Liu, H. and Ong, Y. S. and Shen, X. and Cai, J.},
   title = {When Gaussian Process Meets Big Data: A Review of Scalable GPs},
   journal = {IEEE Transactions on Neural Networks and Learning Systems},
   volume = {31},
   number = {11},
   pages = {4405-4423},
   ISSN = {2162-2388},
   DOI = {10.1109/TNNLS.2019.2957109},
   year = {2020},
   type = {Journal Article}
}

@article{RN818,
   author = {Park, C. and Apley, D.},
   title = {Patchwork Kriging for Large-scale Gaussian Process Regression},
   journal = {Journal of Machine Learning Research},
   volume = {19},
   number = {1},
   pages = {269-311},
   ISSN = {1532-4435},
   url = {<Go to ISI>://WOS:000443222900001},
   year = {2018},
   type = {Journal Article}
}

@misc{RN1479,
   volume = {130},
   pages = {3133--3141},
   url = {http://proceedings.mlr.press/v130/stanton21a.html},
   year = {2021},
   type = {Conference Paper}
}

@article{RN1573,
   author = {Wang, Liwei and Yerramilli, Suraj and Iyer, Akshay and Apley, Daniel and Zhu, Ping and Chen, Wei},
   title = {Scalable Gaussian Processes for Data-Driven Design Using Big Data With Categorical Factors},
   journal = {Journal of Mechanical Design},
   volume = {144},
   number = {2},
   ISSN = {1050-0472},
   DOI = {10.1115/1.4052221},
   url = {https://doi.org/10.1115/1.4052221},
   year = {2021},
   type = {Journal Article}
}



@article{deng2023data,
  title={Data-Driven Calibration of Multifidelity Multiscale Fracture Models Via Latent Map Gaussian Process},
  author={Deng, Shiguang and Mora, Carlos and Apelian, Diran and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  volume={145},
  number={1},
  pages={011705},
  year={2023},
  publisher={American Society of Mechanical Engineers}
}

@article{RN530,
   author = {Bouhlel, Mohamed Amine and Martins, Joaquim RRA},
   title = {Gradient-enhanced kriging for high-dimensional problems},
   journal = {arXiv preprint arXiv:1708.02663},
   year = {2017},
   type = {Journal Article}
}

@article{RN1412,
   author = {Giovanis, Dimitris G. and Shields, Michael D.},
   title = {Data-driven surrogates for high dimensional models using Gaussian process regression on the Grassmann manifold},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {370},
   pages = {113269},
   ISSN = {0045-7825},
   year = {2020},
   type = {Journal Article}
}

@article{RN347,
   author = {Gramacy, Robert B. and Lee, Herbert K. H.},
   title = {Bayesian Treed Gaussian Process Models With an Application to Computer Modeling},
   journal = {Journal of the American Statistical Association},
   volume = {103},
   number = {483},
   pages = {1119-1130},
   ISSN = {0162-1459
1537-274X},
   DOI = {10.1198/016214508000000689},
   url = {<Go to ISI>://WOS:000260193700018},
   year = {2012},
   type = {Journal Article}
}

@article{RN1492,
   author = {Qian, Peter Z. G. and Wu, Huaiqing and Wu, C. F. Jeff},
   title = {Gaussian process models for computer experiments with qualitative and quantitative factors},
   journal = {Technometrics},
   volume = {50},
   number = {3},
   pages = {383-396},
   ISSN = {0040-1706},
   year = {2008},
   type = {Journal Article}
}

@article{RN1214,
   author = {Roustant, Olivier and Padonou, Esperan and Deville, Yves and Clément, Aloïs and Perrin, Guillaume and Giorla, Jean and Wynn, Henry},
   title = {Group kernels for Gaussian process metamodels with categorical inputs},
   journal = {SIAM/ASA Journal on Uncertainty Quantification},
   volume = {8},
   number = {2},
   pages = {775-806},
   ISSN = {2166-2525},
   year = {2020},
   type = {Journal Article}
}

@article{RN713,
   author = {Thimmisetty, Charanraj A. and Ghanem, Roger G. and White, Joshua A. and Chen, Xiao},
   title = {High-Dimensional Intrinsic Interpolation Using Gaussian Process Regression and Diffusion Maps},
   journal = {Mathematical Geosciences},
   volume = {50},
   number = {1},
   pages = {77-96},
   ISSN = {1874-8961
1874-8953},
   DOI = {10.1007/s11004-017-9705-y},
   url = {<Go to ISI>://WOS:000419166200004},
   year = {2017},
   type = {Journal Article}
}

@article{RN1228,
   author = {Tripathy, Rohit and Bilionis, Ilias and Gonzalez, Marcial},
   title = {Gaussian processes with built-in dimensionality reduction: Applications to high-dimensional uncertainty propagation},
   journal = {Journal of Computational Physics},
   volume = {321},
   pages = {191-223},
   ISSN = {0021-9991},
   year = {2016},
   type = {Journal Article}
}

@article{RN321,
   author = {Ulaganathan, S. and Couckuyt, I. and Dhaene, T. and Degroote, J. and Laermans, E.},
   title = {High dimensional Kriging metamodelling utilising gradient information},
   journal = {Applied Mathematical Modelling},
   volume = {40},
   number = {9-10},
   pages = {5256-5270},
   ISSN = {0307904X},
   DOI = {10.1016/j.apm.2015.12.033},
   url = {<Go to ISI>://WOS:000375511900007},
   year = {2016},
   type = {Journal Article}
}

@article{RN1215,
   author = {Zhang, Qiong and Chien, Peter and Liu, Qing and Xu, Li and Hong, Yili},
   title = {Mixed-input Gaussian process emulators for computer experiments with a large number of categorical levels},
   journal = {Journal of Quality Technology},
   pages = {1-11},
   ISSN = {0022-4065
2575-6230},
   DOI = {10.1080/00224065.2020.1778431},
   url = {https://doi.org/10.1080/00224065.2020.1778431},
   year = {2020},
   type = {Journal Article}
}

@article{RN1075,
   author = {Zhang, Yichi and Tao, Siyu and Chen, Wei and Apley, Daniel W.},
   title = {A Latent Variable Approach to Gaussian Process Modeling with Qualitative and Quantitative Factors},
   journal = {Technometrics},
   volume = {62},
   number = {3},
   pages = {291-302},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1080/00401706.2019.1638834},
   url = {<Go to ISI>://WOS:000481877700001},
   year = {2019},
   type = {Journal Article}
}

@article{RN1894,
   author = {Matthews, Alexander G de G and Van Der Wilk, Mark and Nickson, Tom and Fujii, Keisuke and Boukouvalas, Alexis and León-Villagrá, Pablo and Ghahramani, Zoubin and Hensman, James},
   title = {GPflow: A Gaussian Process Library using TensorFlow},
   journal = {J. Mach. Learn. Res.},
   volume = {18},
   number = {40},
   pages = {1-6},
   year = {2017},
   type = {Journal Article}
}

@book{RN332,
   author = {Rasmussen, Carl Edward},
   title = {Gaussian processes for machine learning},
   year = {2006},
   type = {Book}
}
@article{deng2023data,
  title={Data-Driven Calibration of Multifidelity Multiscale Fracture Models Via Latent Map Gaussian Process},
  author={Deng, Shiguang and Mora, Carlos and Apelian, Diran and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  volume={145},
  number={1},
  pages={011705},
  year={2023},
  publisher={American Society of Mechanical Engineers}
}

@article{lee2017deep,
  title={Deep neural networks as gaussian processes},
  author={Lee, Jaehoon and Bahri, Yasaman and Novak, Roman and Schoenholz, Samuel S and Pennington, Jeffrey and Sohl-Dickstein, Jascha},
  journal={arXiv preprint arXiv:1711.00165},
  year={2017}
}
@article{al2017learning,
  title={Learning scalable deep kernels with recurrent structure},
  author={Al-Shedivat, Maruan and Wilson, Andrew Gordon and Saatchi, Yunus and Hu, Zhiting and Xing, Eric P},
  journal={The Journal of Machine Learning Research},
  volume={18},
  number={1},
  pages={2850--2886},
  year={2017},
  publisher={JMLR. org}
}

@article{RN1898,
   author = {Ambikasaran, Sivaram and Foreman-Mackey, Daniel and Greengard, Leslie and Hogg, David W and O’Neil, Michael},
   title = {Fast direct methods for Gaussian processes and the analysis of NASA Kepler mission data},
   journal = {arXiv preprint arXiv:1403.6015},
   year = {2014},
   type = {Journal Article}
}

@article{RN1899,
   author = {Fabian, Pedregosa},
   title = {Scikit-learn: Machine learning in Python},
   journal = {Journal of machine learning research 12},
   pages = {2825},
   year = {2011},
   type = {Journal Article}
}

@article{RN1900,
   author = {Vanhatalo, Jarno and Riihimäki, Jaakko and Hartikainen, Jouni and Jylänki, Pasi and Tolvanen, Ville and Vehtari, Aki},
   title = {GPstuff: Bayesian modeling with Gaussian processes},
   journal = {The Journal of Machine Learning Research},
   volume = {14},
   number = {1},
   pages = {1175-1179},
   ISSN = {1532-4435},
   year = {2013},
   type = {Journal Article}
}

@inproceedings{RN509,
   author = {Azevedo-Filho, Adriano and Shachter, Ross D},
   title = {Laplace's method approximations for probabilistic inferencein belief networks with continuous variables},
   booktitle = {Proceedings of the Tenth international conference on Uncertainty in artificial intelligence},
   publisher = {Morgan Kaufmann Publishers Inc.},
   pages = {28-36},
   ISBN = {1558603328},
   type = {Conference Proceedings}
}

@article{yeom2019performance,
  title={Performance evaluation of automobile fuel consumption using a fuzzy-based granular model with coverage and specificity},
  author={Yeom, Chan-Uk and Kwak, Keun-Chang},
  journal={Symmetry},
  volume={11},
  number={12},
  pages={1480},
  year={2019},
  publisher={MDPI}
}

@article{RN1902,
   author = {Bonilla, Edwin V and Chai, Kian and Williams, Christopher},
   title = {Multi-task Gaussian process prediction},
   journal = {Advances in neural information processing systems},
   volume = {20},
   year = {2007},
   type = {Journal Article}
}

@article{RN328,
   author = {Conti, S. and Gosling, J. P. and Oakley, J. E. and O'Hagan, A.},
   title = {Gaussian process emulation of dynamic computer codes},
   journal = {Biometrika},
   volume = {96},
   number = {3},
   pages = {663-676},
   ISSN = {0006-3444
1464-3510},
   DOI = {10.1093/biomet/asp028},
   url = {<Go to ISI>://WOS:000269196300012},
   year = {2009},
   type = {Journal Article}
}

@article{RN287,
   author = {Conti, Stefano and O’Hagan, Anthony},
   title = {Bayesian emulation of complex multi-output and dynamic computer models},
   journal = {Journal of Statistical Planning and Inference},
   volume = {140},
   number = {3},
   pages = {640-651},
   ISSN = {03783758},
   DOI = {10.1016/j.jspi.2009.08.006},
   url = {<Go to ISI>://WOS:000272635800005},
   year = {2010},
   type = {Journal Article}
}

@article{RN1904,
   author = {Lawrence, Neil},
   title = {Gaussian process latent variable models for visualisation of high dimensional data},
   journal = {Advances in neural information processing systems},
   volume = {16},
   year = {2003},
   type = {Journal Article}
}

@inproceedings{RN1903,
   author = {Titsias, Michalis and Lawrence, Neil D},
   title = {Bayesian Gaussian process latent variable model},
   booktitle = {Proceedings of the thirteenth international conference on artificial intelligence and statistics},
   publisher = {JMLR Workshop and Conference Proceedings},
   pages = {844-851},
   type = {Conference Proceedings}
}

@inproceedings{RN1901,
   author = {Wilson, Andrew Gordon and Hu, Zhiting and Salakhutdinov, Ruslan and Xing, Eric P},
   title = {Deep kernel learning},
   booktitle = {Artificial intelligence and statistics},
   publisher = {PMLR},
   pages = {370-378},
   type = {Conference Proceedings}
}

@article{bingham2018pyro,
author = {Bingham, Eli and Chen, Jonathan P. and Jankowiak, Martin and Obermeyer, Fritz and
          Pradhan, Neeraj and Karaletsos, Theofanis and Singh, Rohit and Szerlip, Paul and
          Horsfall, Paul and Goodman, Noah D.},
title = {{Pyro: Deep Universal Probabilistic Programming}},
journal = {Journal of Machine Learning Research},
year = {2018}
}

@article{RN452,
   author = {Sobol', Il'ya Meerovich},
   title = {On sensitivity estimation for nonlinear mathematical models},
   journal = {Matematicheskoe Modelirovanie},
   volume = {2},
   number = {1},
   pages = {112-118},
   ISSN = {0234-0879},
   year = {1990},
   type = {Journal Article}
}

@article{dixon2023covariance,
  title={Covariance Expressions for Multi-Fidelity Sampling with Multi-Output, Multi-Statistic Estimators: Application to Approximate Control Variates},
  author={Dixon, Thomas O and Warner, James E and Bomarito, Geoffrey F and Gorodetsky, Alex A},
  journal={arXiv preprint arXiv:2310.00125},
  year={2023}
}

@article{RN1770,
   author = {Gorodetsky, A. A. and Jakeman, J. D. and Geraci, G.},
   title = {MFNets: data efficient all-at-once learning of multifidelity surrogates as directed networks of information sources},
   journal = {Computational Mechanics},
   volume = {68},
   number = {4},
   pages = {741-758},
   ISSN = {1432-0924},
   DOI = {10.1007/s00466-021-02042-0},
   url = {https://doi.org/10.1007/s00466-021-02042-0},
   year = {2021},
   type = {Journal Article}
}

@article{RN1876,
   author = {Mora, Carlos and Eweis-Labolle, Jonathan Tammer and Johnson, Tyler and Gadde, Likith and Bostanabad, Ramin},
   title = {Probabilistic neural data fusion for learning from an arbitrary number of multi-fidelity data sets},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {415},
   pages = {116207},
   ISSN = {0045-7825},
   DOI = {https://doi.org/10.1016/j.cma.2023.116207},
   url = {https://www.sciencedirect.com/science/article/pii/S0045782523003316},
   year = {2023},
   type = {Journal Article}
}

@article{RN1845,
   author = {Zanjani Foumani, Zahra and Shishehbor, Mehdi and Yousefpour, Amin and Bostanabad, Ramin},
   title = {Multi-fidelity cost-aware Bayesian optimization},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {407},
   pages = {115937},
   ISSN = {0045-7825},
   DOI = {https://doi.org/10.1016/j.cma.2023.115937},
   url = {https://www.sciencedirect.com/science/article/pii/S0045782523000609},
   year = {2023},
   type = {Journal Article}
}

@article{RN705,
   author = {Kennedy, Marc C and O'Hagan, Anthony},
   title = {Bayesian calibration of computer models},
   journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
   volume = {63},
   number = {3},
   pages = {425-464},
   ISSN = {1467-9868},
   year = {2001},
   type = {Journal Article}
}

@article{RN272,
   author = {Arendt, Paul D. and Apley, Daniel W. and Chen, Wei},
   title = {Quantification of Model Uncertainty: Calibration, Model Discrepancy, and Identifiability},
   journal = {Journal of Mechanical Design},
   volume = {134},
   number = {10},
   pages = {100908},
   ISSN = {1050-0472
1528-9001},
   DOI = {10.1115/1.4007390},
   url = {<Go to ISI>://WOS:000309654400010},
   year = {2012},
   type = {Journal Article}
}

@article{RN271,
   author = {Arendt, Paul D and Apley, Daniel W and Chen, Wei and Lamb, David and Gorsich, David},
   title = {Improving identifiability in model calibration using multiple responses},
   journal = {Journal of Mechanical Design},
   volume = {134},
   number = {10},
   pages = {100909},
   ISSN = {1050-0472},
   year = {2012},
   type = {Journal Article}
}

@article{RN337,
   author = {Bayarri, M. J. and Berger, J. O. and Liu, F.},
   title = {Modularization in Bayesian analysis, with emphasis on analysis of computer
 models},
   journal = {Bayesian Analysis},
   volume = {4},
   number = {1},
   pages = {119-150},
   ISSN = {1936-0975},
   DOI = {10.1214/09-ba404},
   url = {<Go to ISI>://WOS:000273483200008},
   year = {2009},
   type = {Journal Article}
}

@article{RN336,
   author = {Bayarri, M. J. and Walsh, D. and Berger, J. O. and Cafeo, J. and Garcia-Donato, G. and Liu, F. and Palomo, J. and Parthasarathy, R. J. and Paulo, R. and Sacks, J.},
   title = {Computer model validation with functional output},
   journal = {The Annals of Statistics},
   volume = {35},
   number = {5},
   pages = {1874-1906},
   ISSN = {0090-5364},
   DOI = {10.1214/009053607000000163},
   url = {<Go to ISI>://WOS:000251096100002},
   year = {2007},
   type = {Journal Article}
}

@article{RN270,
   author = {Higdon, Dave and Kennedy, Marc and Cavendish, James C. and Cafeo, John A. and Ryne, Robert D.},
   title = {Combining Field Data and Computer Simulations for Calibration and Prediction},
   journal = {SIAM Journal on Scientific Computing},
   volume = {26},
   number = {2},
   pages = {448-466},
   ISSN = {1064-8275
1095-7197},
   DOI = {10.1137/s1064827503426693},
   url = {<Go to ISI>://WOS:000226823100006},
   year = {2004},
   type = {Journal Article}
}

@article{RN334,
   author = {Loeppky, J and Bingham, Derek and Welch, W},
   title = {Computer model calibration or tuning in practice},
   journal = {Technometrics, submitted for publication},
   year = {2006},
   type = {Journal Article}
}

@article{RN335,
   author = {McFarland, John and Mahadevan, Sankaran and Romero, Vicente and Swiler, Laura},
   title = {Calibration and Uncertainty Analysis for Computer Simulations with Multivariate Output},
   journal = {AIAA Journal},
   volume = {46},
   number = {5},
   pages = {1253-1265},
   ISSN = {0001-1452
1533-385X},
   DOI = {10.2514/1.35288},
   url = {<Go to ISI>://WOS:000255493900022},
   year = {2008},
   type = {Journal Article}
}

@article{RN344,
   author = {Qian, Peter Z. G. and Wu, C. F. Jeff},
   title = {Bayesian Hierarchical Modeling for Integrating Low-Accuracy and High-Accuracy Experiments},
   journal = {Technometrics},
   volume = {50},
   number = {2},
   pages = {192-204},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1198/004017008000000082},
   url = {http://dx.doi.org/10.1198/004017008000000082},
   year = {2008},
   type = {Journal Article}
}

@article{RN648,
   author = {Tuo, Rui and Wu, CF},
   title = {Prediction based on the Kennedy-O'Hagan calibration model: asymptotic consistency and other properties},
   journal = {arXiv preprint arXiv:1703.01326},
   year = {2017},
   type = {Journal Article}
}

@article{10.1063/1.4963592,
    author = {Zhang, Weizhao and Ren, Huaqing and Wang, Zequn and Liu, Wing K. and Chen, Wei and Zeng, Danielle and Su, Xuming and Cao, Jian},
    title = "{An integrated computational materials engineering method for woven carbon fiber composites preforming process}",
    journal = {AIP Conference Proceedings},
    volume = {1769},
    number = {1},
    pages = {170036},
    year = {2016},
    month = {10},
    issn = {0094-243X},
    doi = {10.1063/1.4963592},
    url = {https://doi.org/10.1063/1.4963592},
    eprint = {https://pubs.aip.org/aip/acp/article-pdf/doi/10.1063/1.4963592/13727507/170036\_1\_online.pdf},
}
@article{BOTELHO20031843,
title = {Mechanical behavior of carbon fiber reinforced polyamide composites},
journal = {Composites Science and Technology},
volume = {63},
number = {13},
pages = {1843-1855},
year = {2003},
issn = {0266-3538},
doi = {https://doi.org/10.1016/S0266-3538(03)00119-2},
url = {https://www.sciencedirect.com/science/article/pii/S0266353803001192},
author = {E.C Botelho and Ł Figiel and M.C Rezende and B Lauke},
keywords = {Polyamide composites, B. Mechanical properties, C. Elastic properties, D. Fractography},
abstract = {The purpose of this work is to compare tensile, compressive and interlaminar shear properties of different carbon reinforcement/polyamide composites obtained by interfacial polymerization and hot compression molding techniques. Two types of composite matrices were studied: polyamide 6 and polyamide 6/6, both reinforced by fabric and unidirectional carbon fibers. The effects of the fiber volume fraction and the matrix on mechanical properties were analyzed through tensile, interlaminar shear and compressive tests. In general, the results have shown a slight increase of the composite elastic modulus, tensile and compressive strength with the increase of carbon fiber content. The microscopic damage development within selected composites during the loading has been observed through optical and scanning electron microscope techniques and has shown that shear failure at the fiber/matrix interface has been mostly responsible for damage development, initiated at relatively low stress.}
}

@article{RN791,
   author = {Zhang, W. Z. and Bostanabad, R. and Liang, B. and Su, X. M. and Zeng, D. and Bessa, M. A. and Wang, Y. C. and Chen, W. and Cao, J.},
   title = {A numerical Bayesian-calibrated characterization method for multiscale prepreg preforming simulations with tension-shear coupling},
   journal = {Composites Science and Technology},
   volume = {170},
   pages = {15-24},
   ISSN = {0266-3538},
   DOI = {10.1016/j.compscitech.2018.11.019},
   url = {<Go to ISI>://WOS:000456228100003},
   year = {2019},
   type = {Journal Article}
}

@book{RN311,
   author = {Belytschko, Ted and Liu, Wing Kam and Moran, Brian and Elkhodary, Khalil},
   title = {Nonlinear finite elements for continua and structures},
   publisher = {John wiley $\&$ sons},
   ISBN = {1118700082},
   year = {2013},
   type = {Book}
}

@article{RN1854,
   author = {Deng, Shiguang and Apelian, Diran and Bostanabad, Ramin},
   title = {Adaptive spatiotemporal dimension reduction in concurrent multiscale damage analysis},
   journal = {Computational Mechanics},
   ISSN = {1432-0924},
   DOI = {10.1007/s00466-023-02299-7},
   url = {https://doi.org/10.1007/s00466-023-02299-7},
   year = {2023},
   type = {Journal Article}
}

@article{RN1786,
   author = {Deng, Shiguang and Mora, Carlos and Apelian, Diran and Bostanabad, Ramin},
   title = {Data-Driven Calibration of Multifidelity Multiscale Fracture Models Via Latent Map Gaussian Process},
   journal = {Journal of Mechanical Design},
   volume = {145},
   number = {1},
   pages = {1-15},
   ISSN = {1050-0472
1528-9001},
   DOI = {10.1115/1.4055951},
   url = {https://doi.org/10.1115/1.4055951},
   year = {2023},
   type = {Journal Article}
}

@article{RN1655,
   author = {Deng, S. G. and Soderhjelm, C. and Apelian, D. and Bostanabad, R.},
   title = {Reduced-order multiscale modeling of plastic deformations in 3D alloys with spatially varying porosity by deflated clustering analysis},
   journal = {Computational Mechanics},
   pages = {1-32},
   ISSN = {0178-7675},
   DOI = {10.1007/s00466-022-02177-8},
   url = {<Go to ISI>://WOS:000809539000003},
   year = {2022},
   type = {Journal Article}
}

@article{RN1182,
   author = {Gao, Jiaying and Shakoor, Modesar and Domel, Gino and Merzkirch, Matthias and Zhou, Guowei and Zeng, Danielle and Su, Xuming and Liu, Wing Kam},
   title = {Predictive multiscale modeling for Unidirectional Carbon Fiber Reinforced Polymers},
   journal = {Composites Science and Technology},
   volume = {186},
   pages = {107922},
   ISSN = {02663538},
   DOI = {10.1016/j.compscitech.2019.107922},
   url = {<Go to ISI>://WOS:000509630000020},
   year = {2020},
   type = {Journal Article}
}

@article{dvorak1992transformation,
  title={Transformation field analysis of inelastic composite materials},
  author={Dvorak, George J},
  journal={Proceedings of the Royal Society of London. Series A: Mathematical and Physical Sciences},
  volume={437},
  number={1900},
  pages={311--327},
  year={1992},
  publisher={The Royal Society London}
}

@article{roussette2009nonuniform,
  title={Nonuniform transformation field analysis of elastic--viscoplastic composites},
  author={Roussette, Sophie and Michel, Jean-Claude and Suquet, Pierre},
  journal={Composites Science and Technology},
  volume={69},
  number={1},
  pages={22--27},
  year={2009},
  publisher={Elsevier}
}

@article{chakraborty2017surrogate,
  title={A surrogate based multi-fidelity approach for robust design optimization},
  author={Chakraborty, Souvik and Chatterjee, Tanmoy and Chowdhury, Rajib and Adhikari, Sondipon},
  journal={Applied Mathematical Modelling},
  volume={47},
  pages={726--744},
  year={2017},
  publisher={Elsevier}
}
@article{korondi2021multi,
  title={Multi-fidelity design optimisation strategy under uncertainty with limited computational budget},
  author={Korondi, P{\'e}ter Z{\'e}n{\'o} and Marchi, Mariapia and Parussini, Lucia and Poloni, Carlo},
  journal={Optimization and Engineering},
  volume={22},
  pages={1039--1064},
  year={2021},
  publisher={Springer}
}

@article{absi2016multi,
  title={Multi-fidelity approach to dynamics model calibration},
  author={Absi, Ghina N and Mahadevan, Sankaran},
  journal={Mechanical Systems and Signal Processing},
  volume={68},
  pages={189--206},
  year={2016},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%% BO references

@article{brochu2010tutorial,
  title={A tutorial on Bayesian optimization of expensive cost functions, with application to active user modeling and hierarchical reinforcement learning},
  author={Brochu, Eric and Cora, Vlad M and De Freitas, Nando},
  journal={arXiv preprint arXiv:1012.2599},
  year={2010}
}

@article{adams2014tutorial,
  title={A tutorial on Bayesian optimization for machine learning},
  author={Adams, Ryan P},
  journal={Harvard University},
  year={2014}
}

@article{nguyen2023tutorial,
  title={Tutorial on Bayesian optimization},
  author={Nguyen, Loc},
  year={2023},
  publisher={Preprints}
}

@inproceedings{couckuyt2022bayesian,
  title={Bayesian optimization: tutorial},
  author={Couckuyt, Ivo and Gonzalez, Sebastian Rojas and Branke, Juergen},
  booktitle={Proceedings of the Genetic and Evolutionary Computation Conference Companion},
  pages={843--863},
  year={2022}
}

@incollection{frazier2015bayesian,
  title={Bayesian optimization for materials design},
  author={Frazier, Peter I and Wang, Jialei},
  booktitle={Information science for materials discovery and design},
  pages={45--75},
  year={2015},
  publisher={Springer}
}
@inproceedings{turner2021bayesian,
  title={Bayesian optimization is superior to random search for machine learning hyperparameter tuning: Analysis of the black-box optimization challenge 2020},
  author={Turner, Ryan and Eriksson, David and McCourt, Michael and Kiili, Juha and Laaksonen, Eero and Xu, Zhen and Guyon, Isabelle},
  booktitle={NeurIPS 2020 Competition and Demonstration Track},
  pages={3--26},
  year={2021},
  organization={PMLR}
}


%%%%%%%%%%%% GP-based BO
@article{kopsiaftis2019gaussian,
  title={Gaussian process regression tuned by bayesian optimization for seawater intrusion prediction},
  author={Kopsiaftis, George and Protopapadakis, Eftychios and Voulodimos, Athanasios and Doulamis, Nikolaos and Mantoglou, Aristotelis and others},
  journal={Computational intelligence and neuroscience},
  volume={2019},
  year={2019},
  publisher={Hindawi}
}

@article{binois2022survey,
  title={A survey on high-dimensional Gaussian process modeling with application to Bayesian optimization},
  author={Binois, Mickael and Wycoff, Nathan},
  journal={ACM Transactions on Evolutionary Learning and Optimization},
  volume={2},
  number={2},
  pages={1--26},
  year={2022},
  publisher={ACM New York, NY}
}

@inproceedings{sui2018stagewise,
  title={Stagewise safe bayesian optimization with gaussian processes},
  author={Sui, Yanan and Zhuang, Vincent and Burdick, Joel and Yue, Yisong},
  booktitle={International conference on machine learning},
  pages={4781--4789},
  year={2018},
  organization={PMLR}
}
@article{morita2022applying,
  title={Applying Bayesian optimization with Gaussian process regression to computational fluid dynamics problems},
  author={Morita, Yuki and Rezaeiravesh, Saleh and Tabatabaei, Narges and Vinuesa, Ricardo and Fukagata, Koji and Schlatter, Philipp},
  journal={Journal of Computational Physics},
  volume={449},
  pages={110788},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{mcintire2016sparse,
  title={Sparse Gaussian Processes for Bayesian Optimization.},
  author={McIntire, Mitchell and Ratner, Daniel and Ermon, Stefano},
  booktitle={UAI},
  year={2016}
}

@inproceedings{rana2017high,
  title={High dimensional Bayesian optimization with elastic Gaussian process},
  author={Rana, Santu and Li, Cheng and Gupta, Sunil and Nguyen, Vu and Venkatesh, Svetha},
  booktitle={International conference on machine learning},
  pages={2883--2891},
  year={2017},
  organization={PMLR}
}



@article{foumani2023effects,
  title={Safeguarding Multi-fidelity Bayesian Optimization Against Large Model Form Errors and Heterogeneous Noise},
  author={Zanjani Foumani, Zahra and Yousefpour, Amin and Shishehbor, Mehdi and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  pages={1--23},
  year={2023}
}


%%%%%%%%%%%%%%%%%%%%%

@article{RN1917,
   author = {Bernardo, J and Berger, J and Dawid, APAFMS and Smith, A},
   title = {Regression and classification using Gaussian process priors},
   journal = {Bayesian statistics},
   volume = {6},
   pages = {475},
   year = {1998},
   type = {Journal Article}
}

@article{RN1908,
   author = {MacKay, David JC},
   title = {Introduction to Gaussian processes},
   journal = {NATO ASI series F computer and systems sciences},
   volume = {168},
   pages = {133-166},
   ISSN = {0258-1248},
   year = {1998},
   type = {Journal Article}
}

@article{RN292,
   author = {Gramacy, Robert B. and Lee, Herbert K. H.},
   title = {Cases for the nugget in modeling computer experiments},
   journal = {Statistics and Computing},
   volume = {22},
   number = {3},
   pages = {713-722},
   ISSN = {0960-3174
1573-1375},
   DOI = {10.1007/s11222-010-9224-x},
   url = {<Go to ISI>://WOS:000302326400004},
   year = {2010},
   type = {Journal Article}
}

@article{RN1896,
   author = {O'Hagan, A.},
   title = {Curve Fitting and Optimal Design for Prediction},
   journal = {Journal of the Royal Statistical Society: Series B (Methodological)},
   volume = {40},
   number = {1},
   pages = {1-24},
   ISSN = {0035-9246},
   DOI = {https://doi.org/10.1111/j.2517-6161.1978.tb01643.x},
   url = {https://doi.org/10.1111/j.2517-6161.1978.tb01643.x},
   year = {1978},
   type = {Journal Article}
}

% @article{multitaskGP,
%    author={bonilla2007multi},
%   title={Multi-task Gaussian process prediction},
%   author={Bonilla, Edwin V and Chai, Kian and Williams, Christopher},
%   journal={Advances in neural information processing systems},
%   volume={20},
%   year={2007}
% }

% @online{multioutputGP,
%   author = {Gpytorch},
%   title = {ModelList (Multi-Output) GP Regression},
%   url = {https://docs.gpytorch.ai/en/stable/examples/03_Multitask_Exact_GPs/ModelList_GP_Regression.html},
%   journal={Gpytorch}
% }
@article{cover2009comprehensive,
  title={A comprehensive survey of M2AX phase elastic properties},
  author={Cover, MF and Warschkow, O and Bilek, MMM and McKenzie, DR},
  journal={Journal of Physics: Condensed Matter},
  volume={21},
  number={30},
  pages={305403},
  year={2009},
  publisher={IOP Publishing}
}


@inproceedings{foumani2023effects,
  title={Mitigating the Effects of Source-Dependent Bias and Noise on Multi-Source Bayesian Optimization: Application to Materials Design},
  author={Zanjani Foumani, Zahra and Yousefpour, Amin and Shishehbor, Mehdi and Bostanabad, Ramin},
  booktitle={International Design Engineering Technical Conferences and Computers and Information in Engineering Conference},
  volume={87318},
  pages={V03BT03A010},
  year={2023},
  organization={American Society of Mechanical Engineers}
}

@article{carvalho2010horseshoe,
  title={The horseshoe estimator for sparse signals},
  author={Carvalho, Carlos M and Polson, Nicholas G and Scott, James G},
  journal={Biometrika},
  volume={97},
  number={2},
  pages={465--480},
  year={2010},
  publisher={Oxford University Press}
}

@online{BoTorch,
  title = {BoTorch Models},
  author = {Balandat, Maximilian and Karrer, Brian and Jiang, Daniel R. and Daulton, Samuel and Letham, Benjamin and Wilson, Andrew Gordon and Bakshy, Eytan},
  year = {2020},
  url = {https://botorch.org/api/models.html#botorch.models.gp_regression_mixed.MixedSingleTaskGP},
  note = {},
}

@online{Matlab,
  title = {Gaussian Process Regression Models},
  author = {MathWorks},
  year = {2023},
  url = {https://www.mathworks.com/help/stats/gaussian-process-regression-models.html},
  note = {},
}


@book{bishop2006pattern,
  title={Pattern recognition and machine learning},
  author={Bishop, Christopher M and Nasrabadi, Nasser M},
  volume={4},
  number={4},
  year={2006},
  publisher={Springer}
}

@incollection{marelli2014uqlab,
  title={UQLab: A framework for uncertainty quantification in Matlab},
  author={Marelli, Stefano and Sudret, Bruno},
  booktitle={Vulnerability, uncertainty, and risk: quantification, mitigation, and management},
  pages={2554--2563},
  year={2014}
}

@article{saltelli2010variance,
  title={Variance based sensitivity analysis of model output. Design and estimator for the total sensitivity index},
  author={Saltelli, Andrea and Annoni, Paola and Azzini, Ivano and Campolongo, Francesca and Ratto, Marco and Tarantola, Stefano},
  journal={Computer physics communications},
  volume={181},
  number={2},
  pages={259--270},
  year={2010},
  publisher={Elsevier}
}

@article{bracher2021evaluating,
  title={Evaluating epidemic forecasts in an interval format},
  author={Bracher, Johannes and Ray, Evan L and Gneiting, Tilmann and Reich, Nicholas G},
  journal={PLoS computational biology},
  volume={17},
  number={2},
  pages={e1008618},
  year={2021},
  publisher={Public Library of Science San Francisco, CA USA}
}

@article{mitchell2017proper,
  title={Proper scoring rules for interval probabilistic forecasts},
  author={Mitchell, K and Ferro, CAT},
  journal={Quarterly Journal of the Royal Meteorological Society},
  volume={143},
  number={704},
  pages={1597--1607},
  year={2017},
  publisher={Wiley Online Library}
}

@inproceedings{RN1062,
   author = {Mobahi, Hossein and Fisher III, John W},
   title = {A theoretical analysis of optimization by Gaussian continuation},
   booktitle = {Twenty-Ninth AAAI Conference on Artificial Intelligence},
   type = {Conference Proceedings}
}

@article{saves2024smt,
  title={SMT 2.0: A Surrogate Modeling Toolbox with a focus on hierarchical and mixed variables Gaussian processes},
  author={Saves, Paul and Lafage, R{\'e}mi and Bartoli, Nathalie and Diouane, Youssef and Bussemaker, Jasper and Lefebvre, Thierry and Hwang, John T and Morlier, Joseph and Martins, Joaquim RRA},
  journal={Advances in Engineering Software},
  volume={188},
  pages={103571},
  year={2024},
  publisher={Elsevier}
}

@article{halstrup2016black,
  title={Black-box optimization of mixed discrete-continuous optimization problems},
  author={Halstrup, Momchil},
  year={2016}
}

@article{zhou2011simple,
  title={A simple approach to emulation for computer models with qualitative and quantitative factors},
  author={Zhou, Qiang and Qian, Peter ZG and Zhou, Shiyu},
  journal={Technometrics},
  pages={266--273},
  year={2011},
  publisher={JSTOR}
}
@article{saves2023mixed,
  title={A mixed-categorical correlation kernel for Gaussian process},
  author={Saves, Paul and Diouane, Youssef and Bartoli, Nathalie and Lefebvre, Thierry and Morlier, Joseph},
  journal={Neurocomputing},
  pages={126472},
  year={2023},
  publisher={Elsevier}
}
@article{bouhlel2019python,
  title={A Python surrogate modeling framework with derivatives},
  author={Bouhlel, Mohamed Amine and Hwang, John T and Bartoli, Nathalie and Lafage, R{\'e}mi and Morlier, Joseph and Martins, Joaquim RRA},
  journal={Advances in Engineering Software},
  volume={135},
  pages={102662},
  year={2019},
  publisher={Elsevier}
}

@article{bengio2005curse,
  title={The curse of highly variable functions for local kernel machines},
  author={Bengio, Yoshua and Delalleau, Olivier and Roux, Nicolas},
  journal={Advances in neural information processing systems},
  volume={18},
  year={2005}
}

@article{hensman2013gaussian,
  title={Gaussian processes for big data},
  author={Hensman, James and Fusi, Nicolo and Lawrence, Neil D},
  journal={arXiv preprint arXiv:1309.6835},
  year={2013}
}

@article{RN340,
   author = {Ba, Shan and Joseph, V. Roshan},
   title = {Composite Gaussian process models for emulating expensive functions},
   journal = {The Annals of Applied Statistics},
   volume = {6},
   number = {4},
   pages = {1838-1860},
   ISSN = {1932-6157},
   DOI = {10.1214/12-aoas570},
   url = {<Go to ISI>://WOS:000314458400021},
   year = {2012},
   type = {Journal Article}
}
@inproceedings{RN717,
   author = {Le, Quoc V and Smola, Alex J and Canu, Stéphane},
   title = {Heteroscedastic Gaussian process regression},
   booktitle = {Proceedings of the 22nd international conference on Machine learning},
   publisher = {ACM},
   pages = {489-496},
   ISBN = {1595931805},
   type = {Conference Proceedings}
}

@book{murphy2012machine,
  title={Machine learning: a probabilistic perspective},
  author={Murphy, Kevin P},
  year={2012},
  publisher={MIT press}
}


@article{RN607,
  title={Understanding the effects of model uncertainty in robust design with computer experiments},
  author={Apley, Daniel W and Liu, Jun and Chen, Wei},
  year={2006}
}

@article{RN277,
  title={A preposterior analysis to predict identifiability in the experimental calibration of computer models},
  author={Arendt, Paul D and Apley, Daniel W and Chen, Wei},
  journal={IIE Transactions},
  volume={48},
  number={1},
  pages={75--88},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{MLBLUE,
  title={On multilevel best linear unbiased estimators},
  author={Schaden, Daniel and Ullmann, Elisabeth},
  journal={SIAM/ASA Journal on Uncertainty Quantification},
  volume={8},
  number={2},
  pages={601--635},
  year={2020},
  publisher={SIAM}
}

@article{ACV,
  title={A generalized approximate control variate framework for multifidelity uncertainty quantification},
  author={Gorodetsky, Alex A and Geraci, Gianluca and Eldred, Michael S and Jakeman, John D},
  journal={Journal of Computational Physics},
  volume={408},
  pages={109257},
  year={2020},
  publisher={Elsevier}
}

@article{RN295,
   author = {Oakley, J.},
   title = {Bayesian inference for the uncertainty distribution of computer model outputs},
   journal = {Biometrika},
   volume = {89},
   number = {4},
   pages = {769-784},
   ISSN = {0006-3444
1464-3510},
   DOI = {10.1093/biomet/89.4.769},
   url = {<Go to ISI>://WOS:000179774400004},
   year = {2002},
   type = {Journal Article}
}

@article{RN375,
   author = {Plumlee, Matthew},
   title = {Bayesian calibration of inexact computer models},
   journal = {Journal of the American Statistical Association},
   number = {just-accepted},
   ISSN = {0162-1459},
   year = {2016},
   type = {Journal Article}
}

@article{RN377,
   author = {Tuo, Rui and Jeff Wu, C. F.},
   title = {A Theoretical Framework for Calibration in Computer Models: Parametrization, Estimation and Convergence Properties},
   journal = {SIAM/ASA Journal on Uncertainty Quantification},
   volume = {4},
   number = {1},
   pages = {767-795},
   ISSN = {2166-2525},
   DOI = {10.1137/151005841},
   url = {<Go to ISI>://WOS:000407996700030},
   year = {2016},
   type = {Journal Article}
}


==> extera.tex <==

$\operatorname{cov}\left(\xi(\boldsymbol{x}), \xi\left(\boldsymbol{x}^{\prime}\right)\right)=$
The multivariate Gaussian (or Normal) distribution has a joint probability density given by







where $\sigma^{2}$ indicates the variance of the process and the parametric correlation function is represented by $r(.,.)$. Also since $\xi(\boldsymbol{x})$ is a zero-mean GP we have  Also, $\mu(\boldsymbol{x})=\boldsymbol{m}(\boldsymbol{x}) \boldsymbol{\beta}$ where $\boldsymbol{m}(\boldsymbol{x})=\left[m_1(\boldsymbol{x}), \ldots, m_{d\beta}(\boldsymbol{x})\right]$ represents a set of parametric basis functions, $\boldsymbol{\beta} = [\beta_1, \beta_2,..., \beta_{d\beta}]^T$ are unknown coefficients, and $\xi(\boldsymbol{x})$ is a zero-mean GP in which its covariance function or kernel is given by:

%%


\noindent where $\sigma^{2}$ indicates the variance of the process and the parametric correlation function is represented by $r(.,.)$. Also since $\xi(\boldsymbol{x})$ is a zero-mean GP we have 


%%




%=================================================================
\begin{equation} 
    \begin{split}
p(\mathbf{x} \mid \mathbf{m}, \Sigma)=(2 \pi)^{-D / 2}|\Sigma|^{-1 / 2} \exp \left(-\frac{1}{2}(\mathbf{x}-\mathbf{m})^{\top} \Sigma^{-1}(\mathbf{x}-\mathbf{m})\right)
    \end{split}
    \label{eq: joint Gaussian distribution}
\end{equation}
%=================================================================

where $\mathbf{m}$ is the mean vector (of length $D$ ) and $\Sigma$ is the (symmetric, positive definite) covariance matrix (of size $D \times D$ ). As a shorthand we write $\mathbf{x} \sim$ $\mathcal{N}(\mathbf{m}, \Sigma)$

Let $\mathbf{x}$ and $\mathbf{y}$ be jointly Gaussian random vectors




